SHIELD: Suppressing Hallucinations In LVLM Encoders via Bias and Vulnerability Defense

Large Vision-Language Models (LVLMs) excel in diverse cross-modal tasks. However, object hallucination, where models produce plausible but inaccurate object descriptions, remains a significant challenge. In contrast to previous work focusing on LLM components, this paper is the first to trace LVLM hallucinations to visual encoders and identifies three key issues: statistical bias, inherent bias, and vulnerability. To address these challenges, we propose SHIELD, a training-free framework that mitigates hallucinations through three strategies: re-weighting visual tokens to reduce statistical bias, introducing noise-derived tokens to counter inherent bias, and applying adversarial attacks with contrastive decoding to address vulnerability. Experiments demonstrate that SHIELD effectively mitigates object hallucinations across diverse benchmarks and LVLM families. Moreover, SHIELD achieves strong performance on the general LVLM benchmark, highlighting its broad applicability. Code is available at https://github.com/hukcc/SHIELD.

==> figures/inherit-bias.tex <==

\begin{wrapfigure}[12]{r}{2.6in}
\vspace{-14pt}
\centering
\includegraphics[width=1.0\linewidth]{images/module-in-bias-20250814.pdf}  
\caption{Reducing Inherit Bias. $K$ noise inputs are used to estimate the erroneous representations  of dominant objects in the pretraining data, which is subsequently removed from visual tokens through feature subtraction.}
\label{fig:inherit-bias}
\end{wrapfigure}

==> figures/pipeline-multifig.tex <==
\begin{figure*}[t]
    \centering
    \resizebox{1.0\textwidth}{!}{
        \begin{minipage}{0.225\textwidth}
            \begin{subfigure}{\linewidth}
                \centering
                \includegraphics[width=0.85\linewidth]{images/pipeline-1-20250407.pdf}
                \caption{Generate Naive Caption}
                \label{fig:pipelinesub1}
            \end{subfigure}
            \vspace{0.5em}
            \begin{subfigure}{\linewidth}
                \centering
                \includegraphics[width=1.0\linewidth]{images/pipeline-2-20250407.pdf}
                \caption{Calculate Similarity Matrix}
                \label{fig:pipelinesub2}
            \end{subfigure}
            \vspace{0.5em}
            \begin{subfigure}{\linewidth}
                \centering
                \includegraphics[width=1.0\linewidth]{images/pipeline-3-20250407.pdf}
                \caption{Obtain Attack Tensor}
                \label{fig:pipelinesub3}
            \end{subfigure}
        \end{minipage}
        % \hfill
        \hspace{0.7em}
        \begin{minipage}{0.78\textwidth}
            \begin{subfigure}{\linewidth}
                \centering
                \includegraphics[width=1.0\linewidth]{images/pipeline-4-20250407.pdf}
                \caption{CLIP-guided Contrastive Decoding}
                \label{fig:pipelinesub4}
            \end{subfigure}
        \end{minipage}
    }
    \caption{The CCD pipeline begins by generating a naive caption using the vanilla LVLM. A similarity matrix and an attack tensor are then computed via the visual encoder and the paired CLIP text encoder. In the bias reduction process, statistical bias is alleviated by re-weighting visual tokens, thereby preventing overemphasized ones from distorting the perception of fine-grained details. In parallel, inherent bias is estimated using noise inputs, and the corresponding bias-related features are subsequently removed from the visual tokens. In the vulnerability mitigation process, CCD uses the attack tensor to expose vulnerability-induced hallucinations and reduces the probability of generating the related outputs via contrastive decoding.}
    \label{fig:pipeline}
\end{figure*}


==> figures/problem_vis.tex <==
\begin{figure}[t]
    \centering
    \resizebox{0.85\linewidth}{!}{
    \begin{minipage}{0.49\linewidth}
        \begin{subfigure}{\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/ori-att.pdf}
            \caption{Statistical Bias}
            \label{fig:bias-vis-sub1}
        \end{subfigure}
    \end{minipage}
    \begin{minipage}{0.4\linewidth}
        \begin{subfigure}{\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/inherit-bias-Visualization.pdf}
            \caption{Inherent Bias}
            \label{fig:bias-vis-sub2}
        \end{subfigure}
    \end{minipage}
    }
    
    \begin{subfigure}{1.0\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth]{images/Vulnerability.pdf}
        \caption{Vulnerability}
        \label{fig:vulnerability-vis}
    \end{subfigure}
    
    \caption{Statistical bias emphasizes frequent objects, inherent bias induces hallucination tendencies without clear visual cues (e.g., when the input is random noise), and vulnerability causes significant performance drops under small-step attacks (i.e., small perturbations).}
    \label{fig:bias-vis}
\end{figure}


==> figures/problem_vis_hori.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/st-bias-Visualization-20250327.pdf}
        \caption{Statistical Bias: Results from the POPE COCO adversarial split. The X-axis shows the peak-to-average L2 norm ratio among visual tokens; the Y-axis denotes hallucination rate for samples with the same overemphasis level.}
        \label{fig:bias-vis-sub1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/inherit-bias-Visualization-20250324.pdf}
        \caption{Inherent Bias: Results from the POPE COCO subset. The X-axis lists objects; the Y-axis shows hallucination occurrences per object under ambiguous inputs.}
        \label{fig:bias-vis-sub2}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/Vulnerability-20250324.pdf}
        \caption{Vulnerability: Results from the POPE COCO adversarial split. The X-axis is attack steps; the Y-axis is F1 score.}
        \label{fig:vulnerability-vis}
    \end{subfigure}

    \caption{(a) Statistical bias causes frequent visual patterns to be overemphasized, leading to hallucinations. (b) Inherent bias induces erroneous visual representations for frequent objects, especially under ambiguous inputs. (c) Vulnerability makes the model prone to hallucinations under small perturbations.}
    \label{fig:bias-vis}
\end{figure}


==> figures/problem_vul.tex <==
\begin{wrapfigure}[10]{r}{2.8in}
\vspace{-12pt}
    \centering
    \includegraphics[width=1.0\linewidth]{images/Vulnerability-20250908.pdf}
    \caption{Vulnerability makes the model prone to hallucinations under small perturbations.}
    \label{fig:vulnerability-vis}
\end{wrapfigure}


==> figures/st-bias-vis.tex <==
\begin{figure}[t]
    \centering
    \resizebox{0.9\linewidth}{!}{
    \begin{minipage}{0.4\linewidth}
        \begin{subfigure}{\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/st-bias-Visualization.png}
            \caption{Statistical Bias}
            \label{fig:bias-vis-sub1}
        \end{subfigure}
    \end{minipage}
    \begin{minipage}{0.48\linewidth}
        \begin{subfigure}{\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/inherit-bias-Visualization.png}
            \caption{Inherent Bias}
            \label{fig:bias-vis-sub2}
        \end{subfigure}
    \end{minipage}
    }

    \caption{Statistical bias emphasizes frequently occurring objects, while inherent bias causes specific hallucination tendencies, even when the input is random noise.}
    \label{fig:bias-vis}
\end{figure}


==> figures/st-bias.tex <==
\begin{wrapfigure}[11]{r}{2.8in}
\vspace{-12pt}
\centering
\includegraphics[width=1.0\linewidth]{images/module-st-bias-20250814.pdf}  
\caption{
Mitigating Statistical Bias. Visual tokens are re-weighted via a similarity matrix with naive caption tokens, emphasizing more ground-truth-object relevant tokens and reducing overemphasis that distorts fine-grained perception.
}


\label{fig:module-st-bias}
\end{wrapfigure}


==> figures/vulnerability.tex <==
\begin{figure}[t] 
    \centering
    \includegraphics[width=0.9\linewidth]{images/Vulnerability.pdf}  
    \caption{Vulnerability causes errors even with minor input perturbations.}
    \label{fig:vulnerability-vis}
\end{figure}

==> iclr2026/figures/MME-full.tex <==
\begin{wrapfigure}[14]{r}{2.6in}
\vspace{-12pt}
\centering
\includegraphics[width=0.925\linewidth]{images/ridar.pdf}  
\vspace{-10pt}
\caption{Evaluation on the full MME. Larger radar indicate better performance.}
\label{fig:mme-full}
\end{wrapfigure}


==> iclr2026/figures/ablation_vis.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.30\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/ablation-vis-st-bias-20250915.pdf}
        \caption{Token Re-weighting}
        \label{fig:ablation-vis-st-bias}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.35\linewidth}
        \centering
        \includegraphics[width=0.928\linewidth]{images/ablation-vis-in-bias-20250915.pdf}
        \caption{Erroneous Representation Removal}
        \label{fig:ablation-vis-inhernt-bias}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.325\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/ablation-vis-vul-20250915.pdf}
        \caption{Address Vulnerability}
        \label{fig:ablation-vis-vulnerability}
    \end{subfigure}

\vspace{-6pt}
    \caption{(a) Token Re-weighting highlights more object-relevant tokens. (b) Token Subtraction removes erroneous representations, reducing hallucinations associated with dominant objects in the pretraining data. Blue-only categories indicate zero hallucinations with our method. (c) Contrastive Decoding improves robustness to perturbations, mitigating vulnerability-induced hallucinations.}
    \label{fig:ablation-vis}
\vspace{-6pt}
\end{figure}


==> iclr2026/figures/biases-modules.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}[t]{0.53\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/module-st-bias-20250814.pdf}
        \caption{Mitigating Statistical Bias. Visual tokens are re-weighted via a similarity matrix between visual tokens and naive caption tokens, emphasizing more ground-truth-object relevant tokens and reducing overemphasis.}
        \label{fig:module-st-bias}

    \end{minipage}%
    \hfill
    \begin{minipage}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/module-in-bias-20250814.pdf}
        \caption{Reducing Inherent Bias. $K$ noise inputs are used to estimate erroneous representations of dominant objects in the pretraining data, which are then removed from visual tokens via feature subtraction.}
        \label{fig:inherit-bias}

    \end{minipage}
\end{figure}


==> iclr2026/figures/inherit-bias.tex <==

\begin{wrapfigure}[12]{r}{2.6in}
\vspace{-14pt}
\centering
\includegraphics[width=1.0\linewidth]{images/module-in-bias-20250814.pdf}  
\caption{Reducing Inherit Bias. $K$ noise inputs are used to estimate the erroneous representations  of dominant objects in the pretraining data, which is subsequently removed from visual tokens through feature subtraction.}
\label{fig:inherit-bias}
\end{wrapfigure}

==> iclr2026/figures/module-vulnerability.tex <==
\begin{wrapfigure}[14]{r}{3.5in}
\vspace{-16pt}
\centering
\includegraphics[width=1.0\linewidth]{images/module-Vulnerability-20250815.pdf}  
\caption{Addressing Vulnerability. An attack tensor constructed from the input image and its naive caption via adversarial learning is applied to reveal objects likely to be hallucinated, followed by contrastive decoding to suppress their generation.}

\label{fig:module-vulnerability}
\end{wrapfigure}

==> iclr2026/figures/pipeline-multifig.tex <==
\begin{figure*}[t]
    \centering
    \resizebox{1.0\textwidth}{!}{
        \begin{minipage}{0.225\textwidth}
            \begin{subfigure}{\linewidth}
                \centering
                \includegraphics[width=0.85\linewidth]{images/pipeline-1-20250407.pdf}
                \caption{Generate Naive Caption}
                \label{fig:pipelinesub1}
            \end{subfigure}
            \vspace{0.5em}
            \begin{subfigure}{\linewidth}
                \centering
                \includegraphics[width=1.0\linewidth]{images/pipeline-2-20250407.pdf}
                \caption{Calculate Similarity Matrix}
                \label{fig:pipelinesub2}
            \end{subfigure}
            \vspace{0.5em}
            \begin{subfigure}{\linewidth}
                \centering
                \includegraphics[width=1.0\linewidth]{images/pipeline-3-20250407.pdf}
                \caption{Obtain Attack Tensor}
                \label{fig:pipelinesub3}
            \end{subfigure}
        \end{minipage}
        % \hfill
        \hspace{0.7em}
        \begin{minipage}{0.78\textwidth}
            \begin{subfigure}{\linewidth}
                \centering
                \includegraphics[width=1.0\linewidth]{images/pipeline-4-20250407.pdf}
                \caption{CLIP-guided Contrastive Decoding}
                \label{fig:pipelinesub4}
            \end{subfigure}
        \end{minipage}
    }
    \caption{The CCD pipeline begins by generating a naive caption using the vanilla LVLM. A similarity matrix and an attack tensor are then computed via the visual encoder and the paired CLIP text encoder. In the bias reduction process, statistical bias is alleviated by re-weighting visual tokens, thereby preventing overemphasized ones from distorting the perception of fine-grained details. In parallel, inherent bias is estimated using noise inputs, and the corresponding bias-related features are subsequently removed from the visual tokens. In the vulnerability mitigation process, CCD uses the attack tensor to expose vulnerability-induced hallucinations and reduces the probability of generating the related outputs via contrastive decoding.}
    \label{fig:pipeline}
\end{figure*}


==> iclr2026/figures/pipeline.tex <==
\begin{figure*}[t] 
    \centering
    \includegraphics[width=1\linewidth]{images/pipeline-20250910.pdf}  
    \caption{Illustration of the proposed SHIELD framework. Given an input image and a query text, the visual encoder produces tokens affected by statistical bias (overemphasized tokens \includegraphics[height=1.3ex]{images/overemph.png}), inherent bias (erroneous representations \includegraphics[height=1.3ex]{images/errorrep.png}), and vulnerability (inaccurate features \includegraphics[height=1.3ex]{images/inaccuraterep.png}). SHIELD addresses these issues through three modules: (i) \textbf{Token Re-weighting}, which redistributes attention to more ground-truth-object relevant tokens to alleviate overemphasis (\includegraphics[height=1.3ex]{images/overemph.png}); (ii) \textbf{Token Subtraction}, which estimates and removes erroneous representations (\includegraphics[height=1.3ex]{images/errorrep.png}) via noise-derived tokens; and (iii) \textbf{Contrastive Decoding}, which exposes inaccurate features (\includegraphics[height=1.3ex]{images/inaccuraterep.png}) using attacked images and suppresses corresponding outputs by contrasting them with those from the natural image.}
    \label{fig:pipeline}
    \vspace{-14pt}
\end{figure*}

==> iclr2026/figures/problem_bias.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.325\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/prob-st-bias-20250915.pdf}
        \caption{Token Overemphasis}
        \label{fig:bias-vis-sub1}
    \end{subfigure}
    \begin{subfigure}{0.325\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/prob-in-bias-20250915.pdf}
        \caption{Dominant Object Error}
        \label{fig:bias-vis-sub2}
    \end{subfigure}
    \begin{subfigure}{0.325\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/prob-vul-20250915.pdf}
        \caption{Perturbation Vulnerability}
        \label{fig:bias-vis-sub3}
    \end{subfigure}
\vspace{-6pt}
    \caption{Statistics show that hallucinations stem from bias and vulnerability. (a) The X-axis shows the peak-to-average L2 norm ratio of visual tokens, measuring the deviation of the highest-norm token from the average, and the Y-axis shows the proportion of hallucinating samples at each level. Stronger overemphasis leads to higher hallucination rates. (b) The X-axis lists objects, and the Y-axis shows hallucination occurrences under meaningless inputs. Dominant objects are more likely to be falsely perceived as present. (c) The X-axis denotes the number of attack steps, and the Y-axis shows the F1 score. Even small perturbations increase hallucinations and degrade performance.}
    \label{fig:bias-vis}
\vspace{-14pt}
\end{figure}



==> iclr2026/figures/problem_vis.tex <==
\begin{figure}[t]
    \centering
    \resizebox{0.85\linewidth}{!}{
    \begin{minipage}{0.49\linewidth}
        \begin{subfigure}{\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/ori-att.pdf}
            \caption{Statistical Bias}
            \label{fig:bias-vis-sub1}
        \end{subfigure}
    \end{minipage}
    \begin{minipage}{0.4\linewidth}
        \begin{subfigure}{\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/inherit-bias-Visualization.pdf}
            \caption{Inherent Bias}
            \label{fig:bias-vis-sub2}
        \end{subfigure}
    \end{minipage}
    }
    
    \begin{subfigure}{1.0\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth]{images/Vulnerability.pdf}
        \caption{Vulnerability}
        \label{fig:vulnerability-vis}
    \end{subfigure}
    
    \caption{Statistical bias emphasizes frequent objects, inherent bias induces hallucination tendencies without clear visual cues (e.g., when the input is random noise), and vulnerability causes significant performance drops under small-step attacks (i.e., small perturbations).}
    \label{fig:bias-vis}
\end{figure}


==> iclr2026/figures/problem_vis_hori.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/st-bias-Visualization-20250327.pdf}
        \caption{Statistical Bias: Results from the POPE COCO adversarial split. The X-axis shows the peak-to-average L2 norm ratio among visual tokens; the Y-axis denotes hallucination rate for samples with the same overemphasis level.}
        \label{fig:bias-vis-sub1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/inherit-bias-Visualization-20250324.pdf}
        \caption{Inherent Bias: Results from the POPE COCO subset. The X-axis lists objects; the Y-axis shows hallucination occurrences per object under ambiguous inputs.}
        \label{fig:bias-vis-sub2}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/Vulnerability-20250324.pdf}
        \caption{Vulnerability: Results from the POPE COCO adversarial split. The X-axis is attack steps; the Y-axis is F1 score.}
        \label{fig:vulnerability-vis}
    \end{subfigure}

    \caption{(a) Statistical bias causes frequent visual patterns to be overemphasized, leading to hallucinations. (b) Inherent bias induces erroneous visual representations for frequent objects, especially under ambiguous inputs. (c) Vulnerability makes the model prone to hallucinations under small perturbations.}
    \label{fig:bias-vis}
\end{figure}


==> iclr2026/figures/problem_vul.tex <==
\begin{wrapfigure}[10]{r}{2.8in}
\vspace{-12pt}
    \centering
    \includegraphics[width=1.0\linewidth]{images/Vulnerability-20250908.pdf}
    \caption{Vulnerability makes the model prone to hallucinations under small perturbations.}
    \label{fig:vulnerability-vis}
\end{wrapfigure}


==> iclr2026/figures/st-bias-vis.tex <==
\begin{figure}[t]
    \centering
    \resizebox{0.9\linewidth}{!}{
    \begin{minipage}{0.4\linewidth}
        \begin{subfigure}{\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/st-bias-Visualization.png}
            \caption{Statistical Bias}
            \label{fig:bias-vis-sub1}
        \end{subfigure}
    \end{minipage}
    \begin{minipage}{0.48\linewidth}
        \begin{subfigure}{\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/inherit-bias-Visualization.png}
            \caption{Inherent Bias}
            \label{fig:bias-vis-sub2}
        \end{subfigure}
    \end{minipage}
    }

    \caption{Statistical bias emphasizes frequently occurring objects, while inherent bias causes specific hallucination tendencies, even when the input is random noise.}
    \label{fig:bias-vis}
\end{figure}


==> iclr2026/figures/st-bias.tex <==
\begin{wrapfigure}[11]{r}{2.8in}
\vspace{-12pt}
\centering
\includegraphics[width=1.0\linewidth]{images/module-st-bias-20250814.pdf}  
\caption{
Mitigating Statistical Bias. Visual tokens are re-weighted via a similarity matrix with naive caption tokens, emphasizing more ground-truth-object relevant tokens and reducing overemphasis that distorts fine-grained perception.
}


\label{fig:module-st-bias}
\end{wrapfigure}


==> iclr2026/figures/teasor.tex <==
\begin{figure}[b]
\centering
\includegraphics[width=1.0\linewidth]{images/teasor-20250908.pdf}  
\caption{Key issues underlying object hallucinations in LVLMs. Statistical bias: the visual encoder overemphasizes frequent visual patterns, distorting fine-grained perception. Inherent bias: the encoder produces erroneous representations of dominant objects in the pretraining data, regardless of input. Vulnerability: the encoder is sensitive to minor perturbations, yielding unreliable features.}
\label{fig:teasor}
\end{figure}


==> iclr2026/figures/vulnerability.tex <==
\begin{figure}[t] 
    \centering
    \includegraphics[width=0.9\linewidth]{images/Vulnerability.pdf}  
    \caption{Vulnerability causes errors even with minor input perturbations.}
    \label{fig:vulnerability-vis}
\end{figure}

==> iclr2026/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> iclr2026/sections/abstract.tex <==
\begin{abstract}
\label{sec:abstract}
Large Vision-Language Models (LVLMs) excel in diverse cross-modal tasks. However, object hallucination, where models produce plausible but inaccurate object descriptions, remains a significant challenge. In contrast to previous work focusing on LLM components, this paper is the first to trace LVLM hallucinations to visual encoders and identifies three key issues: statistical bias, inherent bias, and vulnerability. To address these challenges, we propose SHIELD, a training-free framework that mitigates hallucinations through three strategies: re-weighting visual tokens to reduce statistical bias, introducing noise-derived tokens to counter inherent bias, and applying adversarial attacks with contrastive decoding to address vulnerability. Experiments demonstrate that SHIELD effectively mitigates object hallucinations across diverse benchmarks and LVLM families. Moreover, SHIELD achieves strong performance on the general LVLM benchmark, highlighting its broad applicability. \textit{Code is available at \url{https://github.com/hukcc/SHIELD}.}
\end{abstract}

==> iclr2026/sections/conclusion.tex <==
\section{Conclusion}
This paper investigates object hallucinations in LVLMs, tracing their origin to visual encoders. Despite large-scale pretraining, these encoders suffer from three issues: statistical bias, which overemphasizes frequent patterns and distorts fine-grained perception; inherent bias, which induces erroneous representations related to dominant objects in pretraining data; and vulnerability, which makes encoders sensitive to minor perturbations and results in inaccurate features. 
To address these challenges, we propose SHIELD, a training-free framework that integrates token re-weighting, token subtraction, and contrastive decoding. Token re-weighting alleviates statistical bias by distributing attention to more ground-truth-relevant tokens. Token subtraction mitigates inherent bias by estimating and removing erroneous dominant-object representations using noise-derived tokens. Contrastive decoding counters vulnerability by exposing hallucinations via perturbed image and suppressing them through contrast with natural inputs. 
Extensive experiments demonstrate that SHIELD not only achieves significant improvements on hallucination benchmarks but also enhances general perception tasks, highlighting its effectiveness and broad applicability.


Future work could explore the design of more robust visual encoders to further reduce bias and vulnerability, as well as the optimization of adversarial attack mechanisms to lower computational costs for real-time applications.

\newpage
\section*{Ethics Statement}
In this paper, we propose SHIELD, a method that mitigates bias and vulnerability to reduce hallucinations in LVLMs, thereby enhancing their safety and reliability for the community. Outputs of SHIELD may occasionally contain inappropriate content inherited from the base model, and such outputs do not reflect the authors' views. We strictly adhere to the ICLR ethical research standards and applicable laws. To the best of our knowledge, this work complies with the General Ethical Principles.



\section*{Reproducibility Statement}
We follow the ICLR reproducibility standards and ensure the reproducibility of our work. All datasets used for inference and evaluation are publicly available, and detailed experimental settings, including hyper-parameters and implementation steps, are documented in the paper and Appendix. Furthermore, we will release our code upon acceptance, enabling other researchers and practitioners to easily reproduce and extend our results.



==> iclr2026/sections/experiments.tex <==
\section{Experiments}
\subsection{Implementation Details}
To evaluate the effectiveness of SHIELD in mitigating hallucinations, three representative LVLMs were selected: LLaVA-1.5 \citep{llava15}, InstructBLIP \citep{instructblip}, and Qwen-VL \citep{qwen-vl}. SHIELD was compared against the corresponding vanilla LVLMs and two recent training-free methods, VCD \citep{VCD} and OPERA \citep{opera_cvpr}. Following their original setups, vanilla LVLMs and VCD adopted sampling-based decoding, while OPERA employed beam search decoding with a penalty term on logits to reduce overconfidence. For SHIELD, sampling-based decoding was used, drawing from the modified post-softmax distribution. Unless otherwise specified, $\alpha=2$, $\beta=0.35$, $K=32$, and $l=0.02$ were applied across all LVLMs, where $\alpha$ controls the strength of contrastive decoding, $\beta$ sets the truncation threshold in the plausibility constraint, $K$ denotes the number of noise inputs for estimating inherent bias, and $l$ is the learning rate for optimizing the attack tensor. Hyper-parameters ablation are provided in the Appendix \ref{app:Hyper-Parameters-Ablation}. All experiments were conducted on a single RTX A6000 GPU.




\subsection{Quantitative Results}
This section evaluates the effectiveness of SHIELD in mitigating hallucinations for both detailed descriptions and simplified VQA answers.

\textbf{CHAIR Evaluation.} 
The CHAIR metric \citep{chair} measures object hallucination in image captioning by calculating the proportion of objects mentioned in captions that are not present in the ground-truth label set. It consists of two dimensions: a sentence-level score $C_S$ and an instance-level score $C_I$, which are defined as:
\begin{equation*}
C_S = \frac{|\text{sentences with hallucinated objects}|}{|\text{all sentences}|},\quad
C_I = \frac{|\text{hallucinated objects}|}{|\text{all objects mentioned}|}.
\end{equation*}
Following \citep{opera_cvpr}, evaluation is performed on 500 randomly selected images from the COCO 2014 validation set \citep{COCO}, using the prompt \textit{``Please describe this image in detail.''} To ensure fairness, generated captions are truncated to a maximum of 512 tokens.


As shown in Table~\ref{table:chair}, SHIELD consistently outperforms all previous training-free methods on both $C_S$ and $C_I$, achieving up to 18\% improvement over the second-best method, OPERA, on LLaVA-1.5. This performance gain stems from SHIELD's ability to counter biases and vulnerability in the visual encoder, thereby reducing hallucination risk in detailed descriptions.


\input{tables/chair-and-GPTaid}

\textbf{GPT-4o Assisted Evaluation.} 
While CHAIR effectively evaluates object-level hallucinations, it fails to capture errors in attributes, locations, or relations. To complement this, we employ GPT-4o, a strong multi-modal assistant, to assess LVLM outputs on the LLaVA-Bench dataset. GPT-4o scores responses on correctness (C) and detailedness (D) from 0–10, with higher correctness indicating fewer hallucinations. The evaluation explicitly targets objects mentioned but absent from the image, as well as errors in attributes, colors, positions, or relationships. Further details are provided in the Appendix \ref{app:GPT-4o-detail}.

As shown in Table~\ref{table:gpt4o-eval}, SHIELD achieves substantial gains in correctness, confirming its effectiveness in mitigating hallucinations. In contrast, improvements in detailedness are modest, since the method primarily addresses bias and vulnerability in the visual encoder rather than enhancing fine-grained descriptive coverage.



\input{tables/POPE-COCO-trainingfree}
\input{tables/MME-trainingfree}
\textbf{POPE Evaluation.} 
Similar to CHAIR, POPE \citep{pope} evaluates existence-level hallucinations in LVLMs. It adopts a VQA-style format (e.g., ``Is there a \{object\} in the image?'') to test whether models correctly associate images with specific objects. POPE includes three splits: ``random'' for random objects, ``popular'' for frequent objects, and ``adversarial'' for objects semantically related to those in the image. The evaluation is conducted on three subsets: COCO, A-OKVQA, and GQA. Additional results are provided in Appendix~\ref{app:more-pope}.

As shown in Table~\ref{table:pope}, SHIELD outperforms previous training-free methods across most splits of the COCO subset. Although all methods show performance drops from Random to Adversarial, SHIELD more effectively mitigates hallucinations in the challenging Adversarial split, highlighting that biases and vulnerability in visual encoders are major contributors to hallucinations. For InstructBLIP, however, the improvements are limited since its Q-Former module constrains the use of modified visual features, thereby diminishing the benefits of SHIELD.


\textbf{MME Hallucination Subset Evaluation.}
Although POPE adopts a VQA format effective for evaluating object-existence-level hallucinations, it does not capture attribute-level aspects such as count, position, and color. To address this limitation, the MME hallucination subsets \citep{MME} provide a more comprehensive benchmark. Following \citep{woodpeaker}, we evaluate object-level hallucinations using the existence and count subsets, and attribute-level hallucinations using the position and color subsets. Performance is reported using the combined metrics of accuracy and accuracy+ as defined in the official implementation.


As shown in Table~\ref{table:mme-hal}, SHIELD achieves consistent improvements across all models, leading to higher total scores. By correcting statistical bias in visual encoders, SHIELD reduces the impact of overemphasized tokens on fine-grained perception, thereby significantly mitigating attribute-level hallucinations.

\input{tables/amber}
\textbf{Attribute and Relation Level Hallucination Evaluation.}
To further evaluate hallucinations at the attribute and relation level, we conduct experiments on the AMBER benchmark~\citep{amber}, comparing against a series of baselines based on LLaVA-1.5 7B. AMBER offers a comprehensive suite of generative and discriminative metrics, explicitly covering existence, attribute, and relation hallucinations, making it a strong benchmark for assessing multimodal hallucination across diverse tasks. As shown in Table~\ref{table:amber}, our method achieves the highest Amber Score (88.0) and consistently outperforms all baselines across most metrics, demonstrating effective mitigation of hallucinations.

\input{tables/mme-and-ablation}
\input{figures/MME-full}
\textbf{LVLM General Evaluation.} 
To evaluate the overall performance of SHIELD-enhanced LVLMs, we conduct experiments on the full MME benchmark \citep{MME} using the LLaVA-1.5 7B model. The benchmark covers ten perception-related subtasks (including four hallucination-related) and four cognition-oriented ones. Performance is reported using both accuracy and accuracy+ as defined in the official implementation.

As shown in Table~\ref{table:mme-full} and Figure~\ref{fig:mme-full}, SHIELD not only improves hallucination-related performance but also yields notable gains in perception tasks such as OCR and Posters, thereby enhancing the overall capability of the model. Further details are provided in the Appendix \ref{app:detail-mme}.




\subsection{Ablation Study}
\textbf{Module Ablation.} 
To assess the effectiveness of SHIELD, we performed ablation studies on each module using the CHAIR benchmark with the LLaVA-1.5 7B model. The adaptive plausibility constraint, a key element of contrastive decoding, was also ablated to evaluate its role in mitigating hallucinations. As shown in Table~\ref{table:ablation}, all modules contribute notably to reducing hallucinations.

Although integral to contrastive decoding, the adaptive plausibility constraint alone was less effective, indicating that filtering low-probability candidates cannot fully suppress hallucinations. In contrast, each SHIELD module individually reduced hallucination frequency, with their full combination achieving the greatest improvement. Notably, after addressing vulnerability, adding the statistical bias mitigation module yielded a further 13\% reduction, highlighting statistical bias as a major source of hallucinations, particularly in longer descriptions.


\input{figures/ablation_vis}
\textbf{Visualization.} 
Figure~\ref{fig:ablation-vis} illustrates SHIELD's effectiveness in mitigating biases and reducing vulnerability in visual encoders. Figure~\ref{fig:ablation-vis-st-bias} demonstrates that re-weighting visual tokens alleviates statistical bias by distributing attention across more object-relevant tokens and reducing overemphasis on specific ones, thereby improving fine-grained perception. Figure~\ref{fig:ablation-vis-inhernt-bias} illustrates SHIELD's effect on the POPE COCO subset with ambiguous inputs, showing that by leveraging noise-derived tokens to remove inaccurate representations, SHIELD significantly reduces hallucinations of dominant objects in pretraining data. Finally, Figure~\ref{fig:ablation-vis-vulnerability} highlights SHIELD's robustness against perturbations, where SHIELD-enhanced LLaVA-1.5 exhibits substantially less performance degradation under increasing attack steps.


\input{tables/infer_cost}
\textbf{Inference Overhead Analysis.} 
To assess the computational cost of SHIELD, we evaluate its hallucination ratio, runtime, and peak GPU memory usage on the CHAIR benchmark with LLaVA-1.5 7B. As shown in Table~\ref{table:chair-efficiency}, SHIELD achieves the lowest hallucination ratio ($C_S$ = 36.6) while maintaining acceptable inference overhead. In particular, it runs substantially faster than OPERA and provides a more favorable trade-off between hallucination reduction and computational efficiency compared to VCD.
To further analyze the sources of computational cost, we conduct a module-wise ablation study using the CHAIR benchmark and LLaVA-1.5 7B, as shown in Table~\ref{table:ablation-modules}. The majority of overhead arises from the Address Vulnerability and Mitigate Statistical Bias modules, both of which require caption generation. In particular, Address Vulnerability further involves adversarial tensor computation, increasing runtime to 7.30 seconds per sample and memory usage to 18.17 GB. The Mitigate Statistical Bias module, which only relies on caption generation, increases runtime to 4.64 seconds and memory to 16.56 GB. For reference, caption generation alone takes 2.05 seconds and 16.56 GB. In contrast, the Reduce Inherent Bias module introduces minimal overhead, adding only 0.04 seconds and 0.81 GB. Notably, the full SHIELD configuration incurs negligible additional cost beyond Address Vulnerability. These results indicate that most overhead is concentrated in caption generation and adversarial tensor computation, and that the overall trade-off can be flexibly adjusted by tuning caption length or the number of adversarial optimization steps.








==> iclr2026/sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}
Large Vision-Language Models (LVLMs) \citep{qwen-vl,llava,instructblip} combine visual and textual information and have advanced significantly in cross-modal tasks. Despite these advances, they suffer from object hallucination, generating object descriptions that may appear reasonable but misrepresent the image, either by misidentifying attributes (e.g., color, quantity, position) or by introducing non-existent objects. This issue poses reliability and safety risks in domains such as healthcare \citep{Advancing,Chatcad}, autonomous systems \citep{Driving,Embodied}, and robotics \citep{LLM,LLM-based}.


\input{figures/teasor}
Various approaches have been proposed to mitigate object hallucinations. Early efforts, such as fine-grained modality alignment \citep{clockonthebeach} and data augmentation to reduce co-occurrence bias \citep{Exposing,chair}, were designed for small-scale VLMs but fail to generalize to LVLMs \citep{Scaling,Emergent}. More recent research falls into two categories: training-required and training-free methods. Training-required methods, including preference optimization \citep{CLIP-DPO}, post-hoc revisers \citep{LURE}, and RLHF \citep{llava-rlhf}, improve factual consistency but demand substantial human and computational resources. In contrast, training-free methods, such as contrasting outputs from distorted inputs \citep{VCD} or applying over-trust penalties during decoding \citep{opera_cvpr}, offer a more efficient alternative. 
However, these approaches primarily focus on the LLM component, leaving the role of visual encoders underexplored. 

This paper is the first to trace LVLM hallucinations to visual encoders, filling this gap by identifying three key issues: statistical bias, inherent bias, and vulnerability, as illustrated in Figure \ref{fig:teasor}. Despite large-scale pretraining, these encoders remain affected by imbalanced distributions of visual concepts in the pretraining data, resulting in statistical and inherent biases. Statistical bias leads the visual encoder to overemphasize tokens related to frequent visual patterns, thereby distorting the perception of details. Inherent bias leads the visual encoder to produce representations of dominant objects in the pretraining data, regardless of the input, even when it is meaningless. Furthermore, vulnerability, arising from insufficient robustness to noise and perturbations during pretraining, leads the encoder to produce inaccurate visual representations even with small perturbations.

To address bias and vulnerability in visual encoders that hinder feature extraction and amplify hallucinations in LVLMs, we propose SHIELD, a training-free method combining token re-weighting, token subtraction, and contrastive decoding. Specifically, token re-weighting alleviates statistical bias by distributing attention across more tokens relevant to the ground-truth objects, thus avoiding fine-grained distortion from overemphasized tokens. In parallel, token subtraction mitigates inherent bias by estimating erroneous representations related to dominant objects in pretraining data via noise input and eliminating them through token-level subtraction. To address vulnerability, contrastive decoding exposes hallucinations with a perturbed image and suppresses them by contrasting with outputs from a natural image.

Experiments demonstrate that SHIELD consistently improves performance on object hallucination benchmarks, including CHAIR \citep{chair}, POPE \citep{pope}, the hallucination subset of MME \citep{MME}, and GPT-4o-aided evaluations on LLaVA-Bench \citep{llava}. Moreover, these improvements are observed across diverse LVLM families, such as LLaVA \citep{llava}, InstructBLIP \citep{instructblip}, and Qwen-VL \citep{qwen-vl}. Beyond object hallucination mitigation, SHIELD also enhances general perception capabilities, as evidenced by improvements on the full MME benchmark \citep{MME}, highlighting its broader applicability.


Our contributions are summarized as follows: 
\begin{itemize}[noitemsep, topsep=0pt, parsep=0pt, partopsep=0pt, leftmargin=*]
\item We analyze the role of visual encoders in contributing to object hallucinations in LVLMs, focusing on statistical bias, inherent bias, and vulnerability.
\item We propose SHIELD, a training-free method that mitigates object hallucinations by reducing statistical bias via token re-weighting, alleviating inherent bias using token subtraction, and addressing vulnerability through contrastive decoding.
\item Comprehensive experiments validate SHIELD's effectiveness in mitigating object hallucinations across diverse benchmarks and LVLM families. Moreover, its strong performance on the general LVLM benchmark highlights its broad applicability.
\end{itemize}

\vspace{-1pt}

==> iclr2026/sections/method.tex <==
\section{Method}
\input{figures/problem_bias}
\subsection{Hallucinations Stem from Visual Encoder}
Accurate visual feature extraction is crucial for LVLMs to generate reliable outputs. However, bias and vulnerability in visual encoders distort features, intensifying object hallucinations. This section delves into these challenges.

\subsubsection{Statistical and Inherent Bias in Visual Encoder} 
\label{bias-define}
Most LVLMs adopt visual encoders derived from pretrained CLIP models. Although these encoders benefit from large-scale pretraining, they are influenced by the imbalanced distribution of visual concepts in the pretraining data. Specifically, certain visual concepts appear far more frequently than others, while rare or context-dependent elements are severely underrepresented \citep{clip-longtailed}. As a result, the model develops a strong inductive bias toward frequent patterns and dominant objects, giving rise to both statistical and inherent bias.

Statistical bias denotes the visual encoder's over-reliance on frequent visual patterns in the pretraining data, causing overemphasis on the corresponding tokens with disproportionately high L2 activation values \citep{L2}. This overemphasis distorts the downstream LLM's perception of fine-grained details by directing attention to overweighted tokens \citep{LLM-att}, often resulting in hallucinations. Analysis of LLaVA-1.5's responses and visual tokens on the POPE COCO subset (Figure~\ref{fig:bias-vis-sub1}) shows that the proportion of hallucinated samples grows with stronger token overemphasis, measured by the peak-to-average L2 ratio (the deviation of the highest-norm token from the mean among visual tokens).

Inherent bias is the visual encoder's overdependence on dominant objects in the pretraining data, leading it to generate erroneous representations of these objects regardless of the input, even when meaningless. As shown in Figure~\ref{fig:bias-vis-sub2}, analysis of LLaVA-1.5's responses to the POPE COCO random split questions with meaningless images (random noise) as input shows frequent hallucinations of dominant objects such as cars, chairs, and tables, defined as cases where the model incorrectly predicts the presence of queried objects.


\subsubsection{Vulnerability in Visual Encoder} 
\label{vulnerability-define}
The vulnerability of visual encoders is another key factor contributing to object hallucinations. It arises from their limited robustness to noise and subtle perturbations \citep{clip-vulnerability}, making them susceptible to constructing inaccurate visual representations under such disturbances. As shown in Figure~\ref{fig:bias-vis-sub3}, the performance of LLaVA-1.5 drops sharply on the POPE COCO subset even with a few attack steps, demonstrating that minor perturbations can exploit this weakness and yield unreliable features.


\input{figures/pipeline}
\subsection{SHIELD: suppressing hallucinations in lvlm encoders via bias and vulnerability defense}

Building on these observations, we propose SHIELD, a training-free method to mitigate object hallucinations by addressing statistical bias, inherent bias, and vulnerability in visual encoders, as illustrated in Figure~\ref{fig:pipeline}. SHIELD integrates three strategies. Token re-weighting distributes attention across more tokens relevant to ground-truth objects, thereby reducing fine-grained distortion from overemphasized tokens and alleviating statistical bias. Token subtraction estimates erroneous representations of dominant objects in the pretraining data using noise input and removes them through token-level subtraction, thus mitigating inherent bias. Finally, contrastive decoding applies perturbations to the input image to expose hallucinations and suppresses them by contrasting outputs with those from the natural image, countering vulnerability.

\subsubsection{Formulation of LVLM Inference}
A LVLM's inference can be described in three stages. First, the visual encoder $E(\cdot)$ extracts $N$ visual tokens from the raw image $\mathbf{v}$:
\begin{equation}
\mathbf{x}^v = {x_0, x_1, \ldots, x_{N-1}} = E(\mathbf{v}).
\end{equation}
Next, given $\mathbf{x}^v$ and the query text $\mathbf{t}$, the LLM computes the output logits for token $y_i$ at step $i$, conditioned on the preceding sequence $y_{<i}$:
\begin{equation}
\operatorname{logit}(y_i \mid \mathbf{x}^v, \mathbf{t}, y_{<i}) = \operatorname{LLM}(\mathbf{x}^v, \mathbf{t}, y_{<i}).
\end{equation}
Finally, the logits are transformed into a probability distribution over the vocabulary via softmax, from which the next token is selected according to the decoding strategy:
\begin{equation}
p(y_i \mid \mathbf{x}^v, \mathbf{t}, y_{<i}) = \operatorname{softmax}\left[\operatorname{logit}(y_i \mid \mathbf{x}^v, \mathbf{t}, y_{<i})\right].
\end{equation}
Autoregressive repetition of the second and third stages produces the final textual output.

\input{figures/biases-modules}
\subsubsection{Mitigating Statistical Bias}
As discussed in Section~\ref{bias-define}, statistical bias causes the visual encoder to overemphasize tokens associated with frequent visual patterns, distorting fine-grained perception. To address this, token re-weighting is applied based on the similarity between visual tokens and naive caption tokens, encouraging the model to attend to more tokens relevant to ground-truth objects.

As shown in Figure~\ref{fig:module-st-bias}, token re-weighting begins with generating a naive caption $\mathbf{c}^{\text{naive}}$ using the vanilla LVLM for the given image $\mathbf{v}$:
\begin{equation}
\mathbf{c}^{\text{naive}} = \operatorname{VanillaLVLM}\big(\mathbf{v}, \textit{``Please describe this image''}\big).
\label{equ:naive-cap}
\end{equation}
The CLIP text encoder $E_t(\cdot)$ (paired with $E(\cdot)$ during CLIP pretraining) then encodes the caption into $P$ tokens:
\begin{equation}
\mathbf{c} = \{c_0, c_1, \ldots, c_{P-1}\} = E_t(\mathbf{c}^{\text{naive}}).
\end{equation}
Given the caption tokens $\mathbf{c}$ and the visual tokens $\mathbf{x}^v$, a similarity matrix $\mathbf{M} \in \mathbb{R}^{N \times P}$ is computed:
\begin{equation}
\mathbf{M}=\frac{\mathbf{x}^v \mathbf{c}^{\top}}{\|\mathbf{x}^v\|_2 \cdot \|\mathbf{c}\|_2}.
\end{equation}
From $\mathbf{M}$, weights $\mathbf{W}^v$ are obtained by taking the maximum along the caption dimension and normalizing to $[0,1]$:
\begin{equation}
\mathbf{W}^v = \operatorname{norm}(\max_j \mathbf{M}_{i,j}), \quad \mathbf{W}^v \in \mathbb{R}^N.
\end{equation}
Finally, the weights are applied via residual addition ($\odot$: element-wise multiplication) to emphasize visual tokens corresponding to captioned objects, yielding statistical-bias-corrected tokens ${\mathbf{x}^v}^\prime$:
\begin{equation}
{\mathbf{x}^v}^{\prime} = {\mathbf{x}^v} + {\mathbf{x}^v} \odot {\mathbf{W}^v}.
\end{equation}
Although the naive caption $\mathbf{c}^{\text{naive}}$ may introduce hallucinations, they do not affect re-weighting, as hallucinated objects fail to match any visual tokens with high similarity during similarity matrix $\mathbf{M}$ computation. Thus, token re-weighting remains focused on ground-truth objects.






\subsubsection{Reducing Inherent Bias} 
As in Section~\ref{bias-define}, inherent bias leads the visual encoder to produce erroneous representations of dominant objects in the pretraining data, regardless of the input. To counter this, token subtraction introduces noise inputs to estimate such erroneous features and removes them from the visual tokens. 


As shown in Figure~\ref{fig:inherit-bias}, $K$ random noise inputs $\mathbf{n}_i$ (with the same size as the image) are passed through the visual encoder. The resulting tokens are averaged to estimate erroneous representations, which are then subtracted from the statistical-bias-corrected tokens ${\mathbf{x}^v}^\prime$, yielding bias-reduced tokens:
\begin{equation}
{\mathbf{x}^v}^{\prime \prime} = {\mathbf{x}^v}^{\prime} - \frac{1}{K} \sum_{i=1}^K E(\mathbf{n}_i).
\end{equation}
Since inherent bias depends only on visual encoder parameters, the estimation of erroneous representations from noise inputs can be pre-calculated for each model to improve efficiency.

The bias-reduced tokens ${\mathbf{x}^v}^{\prime\prime}$, together with the query text $\mathbf{t}$, are subsequently fed into the LLM to produce bias-reduced logits:
\begin{equation}
\operatorname{logit}\left(y_i \mid {\mathbf{x}^v}^{\prime \prime}, \mathbf{t}, y_{<i}\right) = \operatorname{LLM}\left({\mathbf{x}^v}^{\prime \prime}, \mathbf{t}, y_{<i}\right).
\end{equation}



\input{figures/module-vulnerability}
\subsubsection{Address Vulnerability}
\label{sec:method-vuln}
As noted in Section~\ref{vulnerability-define}, the visual encoder lacks robustness to subtle perturbations and noise, making it susceptible to inaccurate representations, especially when key pixels are disturbed. To counter this vulnerability, a two-step strategy is adopted: adversarial attack is first applied to reveal objects likely to be hallucinated, followed by contrastive decoding to suppress the probability of generating the corresponding outputs during inference.


To expose vulnerability-induced hallucinations, an attack tensor is constructed from the input image $\mathbf{v}$ and its naive caption $\mathbf{c}^{\text{naive}}$ (Equation~\ref{equ:naive-cap}) using the visual encoder $E(\cdot)$ and its paired text encoder $E_t(\cdot)$. As illustrated in Figure~\ref{fig:module-vulnerability}, a learnable perturbation $\mathbf{\delta}$ is added to the input image and refined via backpropagation. The adversarial loss is defined as the cosine similarity between the global representation of the perturbed image and that of the naive caption:
\begin{equation}
l_{\text{adv}} = \cos\big(E(\mathbf{v} + \mathbf{\delta}),\; E_t(\mathbf{c}^{\text{naive}})\big).
\end{equation}
The final attack tensor $\mathbf{\delta}^*$ is obtained by minimizing $l_{\text{adv}}$ via gradient descent with learning rate $l$:
\begin{equation}
\mathbf{\delta}^{*} = \arg\min_{\mathbf{\delta}} \; l_{\text{adv}}.
\end{equation}
During inference, the attack tensor $\mathbf{\delta}^*$ is added to the input image to produce vulnerability-induced inaccurate visual representations:
\begin{equation}
\overline{\mathbf{x}}^v = \{\bar{x}_0, \bar{x}_1, \ldots, \bar{x}_{N-1}\} = E(\mathbf{v} + \mathbf{\delta}^*).
\end{equation}
These inaccurate representations are then used to produce adversarial logits:
\begin{equation}
\operatorname{logit}\big(y_i \mid \overline{\mathbf{x}}^v, \mathbf{t}, y_{<i}\big) = \operatorname{LLM}\big(\overline{\mathbf{x}}^v, \mathbf{t}, y_{<i}\big).
\end{equation}
To suppress hallucinations revealed by the attack tensor, contrastive decoding is applied. At each decoding step $i$, SHIELD contrasts the bias-reduced logits with the adversarial logits to adjust the output probability distribution, where $\alpha$ controls the impact of contrastive decoding:
\begin{equation}
p_{shield}(y_i) =
\operatorname{softmax}\!\Big[(1+\alpha)\,\operatorname{logit}(y_i \mid {\mathbf{x}^v}^{\prime\prime}, \mathbf{t}, y_{<i})
- \alpha\,\operatorname{logit}(y_i \mid \overline{\mathbf{x}}^v, \mathbf{t}, y_{<i})\Big],
\end{equation}
Following \citep{VCD}, an adaptive plausibility constraint is introduced to avoid implausible outputs. Only tokens with probabilities no smaller than a fraction $\beta$ of the maximum are retained:
\begin{equation}
\nu_{\text{token}}(y_i) = \{\,y_i \in \nu : p(y_i) \geq \beta \max_{\omega} p(\omega)\,\},
\end{equation}
where $\nu$ is the vocabulary and $\nu_{\text{token}}(y_i)$ is the valid subset at step $i$. The threshold $\beta$ determines truncation aggressiveness. For tokens not in $\nu_{\text{token}}(y_i)$, probabilities are set to zero.





==> iclr2026/sections/related_work.tex <==
\section{Related work}
\subsection{Large Vision Language Models (LVLMs)}
Recent advances in large-scale foundation models and multimodal learning have accelerated the development of Large Vision-Language Models (LVLMs). By combining Large Language Models (LLMs) \citep{Qwen,Learners,vicuna_report,PaLM,ChatGPT,T2Ttransformer,alpaca,Ul2,LLaMA} with cross-modal frameworks such as CLIP \citep{clip} and BLIP \citep{BLIP}, LVLMs integrate visual and textual information for more comprehensive understanding. Nevertheless, LVLMs across different architectures, including LLaVA-1.5 \citep{llava15}, InstructBLIP \citep{instructblip}, and Qwen-VL \citep{qwen-vl}, still suffer from hallucinations, particularly in fine-grained object recognition and challenging visual grounding. Such errors, often involving non-existent objects or misidentified attributes, remain a key challenge for reliability in real-world applications.



\subsection{Object Hallucination in LVLMs} 
Approaches to mitigating object hallucinations in LVLMs can be grouped into training-required and training-free methods. Training-required methods reduce hallucinations by optimizing model parameters or training auxiliary modules. Prominent methods include CLIP-DPO \citep{CLIP-DPO}, leveraging CLIP-based similarity ranking for preference optimization; LURE \citep{LURE}, using post-hoc revisers to align text with visual input; and LLaVA-RLHF \citep{llava-rlhf}, incorporating human feedback through reinforcement learning. Training-free methods improve decoding without modifying model. Representative approaches include Visual Contrastive Decoding (VCD) \citep{VCD}, which contrasts outputs from natural and blur inputs to mitigate hallucinations, OPERA \citep{opera_cvpr}, which reduces overconfidence through penalty mechanisms and token-level adjustments, HALC \citep{HALC}, which employs adaptive focal-contrast decoding to provide token-wise visual grounding during inference, MARINE \citep{MARINE}, which incorporates image-grounded guidance from external vision models, and VTI \citep{VTI}, which steers latent representations to stabilize vision features at test time.  
While effective, these methods rarely address the bias and vulnerability of visual encoders, which this work aims to address.



==> iclr2026/tables/CHAIR-trainingfree.tex <==
% \begingroup
% \begin{table}[t]
% % \renewcommand{\arraystretch}{1.1}  
% \renewcommand{\arraystretch}{1.0}  
% % \small
% \centering
% \caption{Comparison with Training-Free Methods on CHAIR}
% \begin{tabular}{ccccccc}
% \toprule
%                          & \multicolumn{2}{c}{LLaVA-1.5} & \multicolumn{2}{c}{InstructBLIP} & \multicolumn{2}{c}{Qwen-VL} \\
% \multirow{-2}{*}{Method} & $C_S$$\downarrow$  & $C_I$$\downarrow$   & $C_S$$\downarrow$        & $C_I$$\downarrow$       & $C_S$$\downarrow$     & $C_I$$\downarrow$     \\ \hline
% Vanilla                  & 48.8                 & 14.2                  & 54.6                       & 24.8                      & 49.2                    & 13.1         \\
% VCD                      & 46.8                 & 13.2                  & 44.0                       & 13.6                      & 46.4                    & 11.9         \\
% OPERA                    & 44.6                 & 12.8                  & 46.4                       & 14.2                      & 34.6                    & 9.5          \\
% \rowcolor[HTML]{C0C0C0} 
% CCD (Ours)                     & \textbf{36.6} & \textbf{10.3} & \textbf{40.4}   & \textbf{10.9}  & \textbf{28.9}            & \textbf{9.2}             \\ 
% \bottomrule
% \end{tabular}
% \label{table:chair}
% \end{table}
% \endgroup


==> iclr2026/tables/GPT4o-aid-eval.tex <==
\begingroup
\renewcommand{\arraystretch}{1.0}  
\begin{table}[t]
\centering
\caption{GPT-4o Assisted Hallucination Evaluation}
\begin{tabular}{ccccccc}
\toprule
                         & \multicolumn{2}{c}{LLaVA-1.5}        & \multicolumn{2}{c}{InstructBLIP}      & \multicolumn{2}{c}{Qwen-VL} \\
\multirow{-2}{*}{Method} & $C$$\uparrow$    & $D$$\uparrow$     & $C$$\uparrow$     & $D$$\uparrow$     & $C$$\uparrow$ & $D$$\uparrow$ \\ \hline
Vanilla                  & 4.9              & 5.0               & 4.2               & 4.2               &  6.2             & 4.6              \\
VCD                      & 5.5              & 5.5               & 5.1               & \textbf{5.5}      &  6.5             & 5.7              \\
OPERA                    & 5.6              & 6.0               & 5.3               & 5.2               &  6.5             & 5.6                  \\
\rowcolor[HTML]{C0C0C0} 
CCD (Ours)                      & \textbf{6.2}     & \textbf{6.1}      & \textbf{5.6}      & 5.3               &  \textbf{6.9}    & \textbf{5.8}              \\ 
\bottomrule
\end{tabular}
\label{table:gpt4o-eval}
\end{table}
\endgroup


==> iclr2026/tables/MME-full.tex <==
\begin{table}[t]
\centering

\caption{LVLM General Evaluation on MME Dataset}
\begin{tabular}{cccc}
\toprule
Method  & Perception$\uparrow$       & Cognition$\uparrow$       & Total Score$\uparrow$     \\ \hline
Vanilla & 1279.2           & 352.9           & 1632.1          \\
VCD     & 1363.9           & \textbf{353.2}  & 1717.1          \\
OPERA   & 1413.0           & 304.2           & 1717.2          \\
\rowcolor[HTML]{C0C0C0} 
CCD (Ours)    & \textbf{1473.0}  & 337.8           & \textbf{1810.8} \\ \bottomrule
\end{tabular}
\label{table:mme-full}
\end{table}


==> iclr2026/tables/MME-trainingfree.tex <==
\begingroup
\begin{table}[t]
\centering

\scriptsize
\caption{MME Hallucination Evaluation}
\vspace{-6pt}
\begin{tabular}{cc|cccc|c}
\toprule
                               &                              & \multicolumn{2}{c}{Object-level}                                         & \multicolumn{2}{c|}{Attribute-level}                                      &                                         \\ \cline{3-6}
\multirow{-2}{*}{LVLM}         & \multirow{-2}{*}{Method}     & Existence Score $\uparrow$                             & Count Score $\uparrow$                        & Position Score $\uparrow$                     & Color Score $\uparrow$                                 & \multirow{-2}{*}{Total Score $\uparrow$}                 \\ \hline
                               & Vanilla                      & 175.6                                  & 124.6                         & 114.0                         & 151.0                                  & 565.3                                  \\
                               & VCD                          & 184.6                                  & 138.3                & 128.6                & 153.0                                  & 604.6                                  \\
                               & OPERA                        & 180.6                                  & 133.3                         & 123.3                         & 155.0                                  & 592.3                                  \\
\multirow{-4}{*}{LLaVA-1.5}    & \cellcolor[HTML]{C0C0C0}Ours & \cellcolor[HTML]{C0C0C0}\textbf{195.0} & \cellcolor[HTML]{C0C0C0}\textbf{141.6} & \cellcolor[HTML]{C0C0C0}\textbf{148.3} & \cellcolor[HTML]{C0C0C0}\textbf{183.3} & \cellcolor[HTML]{C0C0C0}\textbf{668.3} \\ \hline
                               & Vanilla                      & 141.0                                  & 75.3                          & 66.6                          & 97.3                                   & 380.3                                  \\
                               & VCD                          & 168.3                                  & \textbf{92.3}                          & 64.0                          & 123.0                                  & 447.6                                  \\
                               & OPERA                        & 156.0                                  & 78.3                          & 55.0                          & 95.0                                   & 384.3                                  \\
\multirow{-4}{*}{InstructBLIP} & \cellcolor[HTML]{C0C0C0}Ours & \cellcolor[HTML]{C0C0C0}\textbf{170.0}                & \cellcolor[HTML]{C0C0C0}75.0      & \cellcolor[HTML]{C0C0C0}\textbf{88.3}      & \cellcolor[HTML]{C0C0C0}\textbf{128.3}               & \cellcolor[HTML]{C0C0C0}\textbf{461.6}               \\ \hline
                               & Vanilla                      & 155.0                                  & 127.6                         & 131.6                         & 173.0                                  & 587.3                                  \\
                               & VCD                          & 156.0                                  & 131.0                         & 128.0                         & 181.6                                  & 596.6                                  \\
                               & OPERA                        & 165.0                                  & 145.0                         & \textbf{133.3}                         & 180.0                                  & 623.3                                  \\
\multirow{-4}{*}{Qwen-VL}      & \cellcolor[HTML]{C0C0C0}Ours & \cellcolor[HTML]{C0C0C0}\textbf{180.0}                & \cellcolor[HTML]{C0C0C0}\textbf{170.0}       & \cellcolor[HTML]{C0C0C0}128.3       & \cellcolor[HTML]{C0C0C0}\textbf{190.0}               & \cellcolor[HTML]{C0C0C0}\textbf{668.3}               \\ \bottomrule
\end{tabular}
\vspace{-14pt}
\label{table:mme-hal}
\end{table}
\endgroup


==> iclr2026/tables/MMhal.tex <==
\begin{table}[t]
\centering
\scriptsize
\renewcommand{\arraystretch}{1.0}
\caption{MMHal-Bench Evaluation (LLaVA-1.5 7B)}
\vspace{-4pt}

{\color{blue}
\begin{tabular}{lcccccccccc}
\toprule
\textbf{Method} &
\textbf{Overall}$\uparrow$ &
\textbf{Hallucination}$\downarrow$ &
\textbf{Attribute}$\uparrow$ &
\textbf{Adversarial}$\uparrow$ &
\textbf{Comparison}$\uparrow$ &
\textbf{Counting}$\uparrow$ &
\textbf{Relation}$\uparrow$ &
\textbf{Environment}$\uparrow$ &
\textbf{Holistic}$\uparrow$ &
\textbf{Other}$\uparrow$ \\
\midrule

Vanilla 
& 2.21 
& 0.70 
& \textbf{2.75}
& \textbf{2.00}
& 2.50
& 2.50
& 1.67
& 2.17
& 1.83
& 2.25 \\

\rowcolor[HTML]{C0C0C0}
Ours    
& \textbf{2.65}
& \textbf{0.61}
& 2.42
& 1.83
& \textbf{2.58}
& \textbf{2.67}
& \textbf{2.83}
& \textbf{3.92}
& \textbf{2.08}
& \textbf{2.83} \\

\bottomrule
\end{tabular}
}
\end{table}


==> iclr2026/tables/POPE-COCO-trainingfree.tex <==
\begingroup
\begin{table}[t]
\centering
\scriptsize
\caption{POPE Hallucination Evaluation on COCO subset}
\vspace{-6pt}
\begin{tabular}{cc|cccccc|cc}
\toprule
                               & \multicolumn{1}{c|}{}                           & \multicolumn{2}{c}{Random}                                                    & \multicolumn{2}{c}{Popular}                                                   & \multicolumn{2}{c|}{Adversarial}                                              & \multicolumn{2}{c}{Average}                                                    \\ \cline{3-10} 
\multirow{-2}{*}{LVLM}         & \multicolumn{1}{c|}{\multirow{-2}{*}{Method}} & Accuracy $\uparrow$                                  & F1 $\uparrow$                                   & Accuracy $\uparrow$                                  & F1 $\uparrow$                                   & Accuracy $\uparrow$                                  & F1 $\uparrow$                                   & Accuracy $\uparrow$                                   & F1 $\uparrow$                                   \\ \hline
                               & Vanilla                                         & 83.2                                  & 81.3                                  & 81.8                                  & 80.0                                  & 78.9                                  & 77.5                                  & 81.3                                   & 79.6                                  \\
                               & VCD                                             & 87.7                                  & 87.1                                  & 85.3                                  & 85.0                                  & 80.8                                  & 81.3                                  & 84.6                                   & 84.4                                  \\
                               & OPERA                                           & 89.1                                  & 89.0                                  & 86.0                                  & 86.3                                  & 79.1                                  & 80.9                                  & 84.7                                   & 85.4                                  \\
\multirow{-4}{*}{LLaVA-1.5}    & \cellcolor[HTML]{C0C0C0}Ours                   & \cellcolor[HTML]{C0C0C0}\textbf{91.3} & \cellcolor[HTML]{C0C0C0}\textbf{91.1} & \cellcolor[HTML]{C0C0C0}\textbf{87.4} & \cellcolor[HTML]{C0C0C0}\textbf{87.6} & \cellcolor[HTML]{C0C0C0}\textbf{82.5} & \cellcolor[HTML]{C0C0C0}\textbf{83.6} & \cellcolor[HTML]{C0C0C0}\textbf{87.0}  & \cellcolor[HTML]{C0C0C0}\textbf{87.4} \\ \hline
                               & Vanilla                                         & 80.7                                  & 80.4                                  & 78.2                                  & 78.3                                  & 75.8                                  & 76.5                                  & 78.2                                   & 78.4                                  \\
                               & VCD                                             & 84.5                                  & 83.6                                  & 81.4                                  & 81.0                                  & 79.5                                  & 79.5                                  & 81.8                                   & 81.3                                  \\
                               & OPERA                                           & \textbf{89.8}                         & \textbf{89.6}                         & 83.4                                  & 84.0                                  & 80.7                                  & 81.8                                  & 84.6                                   & \textbf{85.1}                         \\
\multirow{-4}{*}{InstructBLIP} & \cellcolor[HTML]{C0C0C0}Ours                    & \cellcolor[HTML]{C0C0C0}88.2          & \cellcolor[HTML]{C0C0C0}87.6          & \cellcolor[HTML]{C0C0C0}\textbf{84.6} & \cellcolor[HTML]{C0C0C0}\textbf{84.3} & \cellcolor[HTML]{C0C0C0}\textbf{82.2} & \cellcolor[HTML]{C0C0C0}\textbf{82.4} & \cellcolor[HTML]{C0C0C0}\textbf{85.0}  & \cellcolor[HTML]{C0C0C0}84.8          \\ \hline
                               & Vanilla                                         & 84.7                                  & 82.6                                  & 84.1                                  & 82.0                                  & 82.2                                  & 80.3                                  & 83.6                                   & 81.6                                  \\
                               & VCD                                             & 88.6                                  & 87.8                                  & 87.1                                  & 86.4                                  & 84.2                                  & 83.9                                  & 86.6                                   & 86.0                                  \\
                               & OPERA                                           & 86.1                                  & 84.2                                  & 85.7                                  & 83.8                                  & 83.9                                  & 82.1                                  & 85.2                                   & 83.3                                  \\
\multirow{-4}{*}{Qwen-VL}      & \cellcolor[HTML]{C0C0C0}Ours                    & \cellcolor[HTML]{C0C0C0}\textbf{89.2} & \cellcolor[HTML]{C0C0C0}\textbf{88.6} & \cellcolor[HTML]{C0C0C0}\textbf{87.6} & \cellcolor[HTML]{C0C0C0}\textbf{87.1} & \cellcolor[HTML]{C0C0C0}\textbf{84.3} & \cellcolor[HTML]{C0C0C0}\textbf{84.2} & \cellcolor[HTML]{C0C0C0}\textbf{87.0} & \cellcolor[HTML]{C0C0C0}\textbf{86.6} \\
\bottomrule
\end{tabular}

\vspace{-6pt}
\label{table:pope}
\end{table}
\endgroup


==> iclr2026/tables/POPE-traingfree.tex <==
\begingroup
\begin{table*}[ht]
\centering
\label{table:pope}
\begin{tabular}{ccl|cccccc|cc}
\toprule
                                &                           & \multicolumn{1}{c}{}                           & \multicolumn{2}{c}{Random}                                                    & \multicolumn{2}{c}{Popular}                                                   & \multicolumn{2}{c}{Adversarial}                                               & \multicolumn{2}{c}{Average}                                                   \\
\cline{4-5} \cline{6-7} \cline{8-9} \cline{10-11}
                                
\multirow{-2}{*}{LVLM}          & \multirow{-2}{*}{Dataset} & \multicolumn{1}{c}{\multirow{-2}{*}{Method}} & Acc$\uparrow$                                  & F1$\uparrow$                                   & Acc$\uparrow$                                  & F1$\uparrow$                                   & Acc$\uparrow$                                  & \multicolumn{1}{c}{F1$\uparrow$}                                   & Acc$\uparrow$                                  & F1$\uparrow$                                   \\
\cline{1-11}
                                &                           & Vanilla\cite{llava}                                        & 83.2                                  & 81.3                                  & 81.8                                  & 80.0                                  & 78.9                                  & 77.5                                  & 81.3                                  & 79.6                                  \\
                                &                           & VCD\cite{VCD}                                            & 87.7                                  & 87.1                                  & 85.3                                  & 85.0                                  & 80.8                                  & 81.3                                  & 84.6                                  & 84.4                                  \\
                                &                           & OPERA\cite{OPERA}                                          & 89.1                                  & 89.0                                  & 86.0                                  & 86.3                                  & 79.1                                  & 80.9                                  & 84.7                                  & 85.4                                  \\
                                & \multirow{-4}{*}{COCO}    & \cellcolor[HTML]{C0C0C0}Ours                   & \cellcolor[HTML]{C0C0C0}\textbf{91.3} & \cellcolor[HTML]{C0C0C0}\textbf{91.1} & \cellcolor[HTML]{C0C0C0}\textbf{87.4} & \cellcolor[HTML]{C0C0C0}\textbf{87.6} & \cellcolor[HTML]{C0C0C0}\textbf{82.5} & \cellcolor[HTML]{C0C0C0}\textbf{83.6} & \cellcolor[HTML]{C0C0C0}\textbf{87.0} & \cellcolor[HTML]{C0C0C0}\textbf{87.4} \\
\cline{1-11}
                                &                           & Vanilla\cite{instructblip}                                        & 80.7                                  & 80.4                                  & 78.2                                  & 78.3                                  & 75.8                                  & 76.5                                  & 78.2                                  & 78.4                                  \\
                                &                           & VCD\cite{VCD}                                            & 84.5                                  & 83.6                                  & 81.4                                  & 81.0                                  & 79.5                                  & 79.5                                  & 81.8                                  & 81.3                                  \\
                                &                           & OPERA\cite{OPERA}                                          & \textbf{89.8}                         & \textbf{89.6}                         & 83.4                                  & 84.0                                  & 80.7                                  & 81.8                                  & 84.6                                  & \textbf{85.1}                         \\
                                & \multirow{-4}{*}{COCO}    & \cellcolor[HTML]{C0C0C0}Ours                   & \cellcolor[HTML]{C0C0C0}88.6          & \cellcolor[HTML]{C0C0C0}88.0          & \cellcolor[HTML]{C0C0C0}\textbf{84.9} & \cellcolor[HTML]{C0C0C0}\textbf{84.6} & \cellcolor[HTML]{C0C0C0}\textbf{81.8} & \cellcolor[HTML]{C0C0C0}\textbf{82.1} & \cellcolor[HTML]{C0C0C0}\textbf{85.1} & \cellcolor[HTML]{C0C0C0}84.9          \\
\cline{1-11}
                                &                           & Vanilla\cite{qwen-vl}                                        & 84.7                                  & 82.6                                  & 84.1                                  & 82.0                                  & 82.2                                  & 80.3                                  & 83.6                                  & 81.6                                  \\
                                &                           & VCD\cite{VCD}                                            & 88.6                                  & 87.8                                  & 87.1                                  & 86.4                                  & 84.2                                  & 83.9                                  & 86.6                                  & 86.0                                  \\
                                &                           & OPERA\cite{OPERA}                                          & 86.1                                  & 84.2                                  & 85.7                                  & 83.8                                  & 83.9                                  & 82.1                                  & 85.2                                  & 83.3                                  \\
                                & \multirow{-4}{*}{COCO}    & \cellcolor[HTML]{C0C0C0}Ours                   & \cellcolor[HTML]{C0C0C0}              & \cellcolor[HTML]{C0C0C0}              & \cellcolor[HTML]{C0C0C0}              & \cellcolor[HTML]{C0C0C0}              & \cellcolor[HTML]{C0C0C0}              & \cellcolor[HTML]{C0C0C0}              & \cellcolor[HTML]{C0C0C0}              & \cellcolor[HTML]{C0C0C0}              \\ 
\bottomrule
\end{tabular}
\caption{Comparison with Training-Free Methods on POPE}
\end{table*}
\endgroup


==> iclr2026/tables/amber.tex <==
\begingroup
\begin{table}[t]
\centering
\scriptsize
\caption{AMBER Hallucination Evaluation}
\vspace{-6pt}

\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{4}{c}{\textbf{Generative Task}} &
\multicolumn{4}{c}{\textbf{Discriminative Task}} &
\multirow{2}{*}{\shortstack{\textbf{AMBER}\\\textbf{Score}}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
& CHAIR$\downarrow$ & Cover$\uparrow$ & Hallucination$\downarrow$ & Cognition$\downarrow$
& Accuracy$\uparrow$ & Precision$\uparrow$ & Recall$\uparrow$ & F1$\uparrow$
& \\ 
\midrule

Vanilla & 9.2 & 41.3 & 29.2 & 3.7 & 65.7 & 83.2 & 64.7 & 73.2 & 82.0 \\
VCD     & 8.1 & 44.2 & 28.6 & 3.1 & 68.3 & 85.8 & 65.2 & 74.0 & 82.9 \\
OPERA   & 8.3 & 43.1 & 31.2 & 2.9 & 76.0 & 79.2 & \textbf{83.8} & 81.4 & 86.5 \\
\rowcolor[HTML]{C0C0C0}
Ours    & \textbf{6.4} & \textbf{46.1} & \textbf{25.1} & \textbf{1.8}
        & \textbf{78.3} & \textbf{89.1} & 76.6 & \textbf{82.4} & \textbf{88.0} \\
\bottomrule
\end{tabular}
\label{table:amber}
\vspace{-6pt}
\end{table}
\endgroup


==> iclr2026/tables/chair-and-GPTaid.tex <==
\begingroup
\begin{table}[t]
    \centering
    \begin{minipage}{0.52\textwidth}
        \centering
        \scriptsize
        \caption{CHAIR Hallucination Evaluation}
        \begin{tabular}{ccccccc}
        \toprule
                             & \multicolumn{2}{c}{LLaVA-1.5} & \multicolumn{2}{c}{InstructBLIP} & \multicolumn{2}{c}{Qwen-VL} \\
        \multirow{-2}{*}{Method} & $C_S$$\downarrow$  & $C_I$$\downarrow$   & $C_S$$\downarrow$        & $C_I$$\downarrow$       & $C_S$$\downarrow$     & $C_I$$\downarrow$     \\ \hline
        Vanilla                  & 48.8 & 14.2 & 54.6 & 24.8 & 49.2 & 13.1 \\
        VCD                      & 46.8 & 13.2 & 44.0 & 13.6 & 46.4 & 11.9 \\
        OPERA                    & 44.6 & 12.8 & 46.4 & 14.2 & 34.6 & 9.5 \\
        \rowcolor[HTML]{C0C0C0} 
        Ours               & \textbf{36.6} & \textbf{10.3} & \textbf{40.4} & \textbf{10.9} & \textbf{28.9} & \textbf{9.2} \\ 
        \bottomrule
        \end{tabular}
        \label{table:chair}
\vspace{-10pt}
    \end{minipage}\hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \scriptsize
        \caption{GPT4o-aid Hallucination Evaluation}
        \begin{tabular}{ccccccc}
        \toprule
                             & \multicolumn{2}{c}{LLaVA-1.5} & \multicolumn{2}{c}{InstructBLIP} & \multicolumn{2}{c}{Qwen-VL} \\
        \multirow{-2}{*}{Method} & $C$$\uparrow$ & $D$$\uparrow$ & $C$$\uparrow$ & $D$$\uparrow$ & $C$$\uparrow$ & $D$$\uparrow$ \\ \hline
        Vanilla                  & 4.9 & 5.0 & 4.2 & 4.2 & 6.2 & 4.6 \\
        VCD                      & 5.5 & 5.5 & 5.1 & \textbf{5.5} & 6.5 & 5.7 \\
        OPERA                    & 5.6 & 6.0 & 5.3 & 5.2 & 6.5 & 5.6 \\
        \rowcolor[HTML]{C0C0C0} 
        Ours               & \textbf{6.2} & \textbf{6.1} & \textbf{5.6} & 5.3 & \textbf{6.9} & \textbf{5.8} \\ 
        \bottomrule
        \end{tabular}
        \label{table:gpt4o-eval}
\vspace{-10pt}
    \end{minipage}
\end{table}
\endgroup


==> iclr2026/tables/infer_cost.tex <==
\begin{table}[t]
\centering
\begin{minipage}{0.48\linewidth}
\renewcommand{\arraystretch}{1.0}  
    \centering
    \scriptsize
    \caption{Efficiency Comparison on CHAIR}
\vspace{-6pt}

    \begin{tabular}{lccc}
    \toprule
    Method  & $C_S$$\downarrow$ & T (s/sample)$\downarrow$ & Mem$\downarrow$ \\ \hline
    Vanilla & 48.8      & 2.59   & 15.69GB \\
    VCD     & 46.8      & 4.89   & 16.52GB \\
    OPERA   & 44.6      & 24.01  & 34.88GB \\
    \rowcolor[HTML]{C0C0C0}
    Ours    & \textbf{36.6} & 7.34   & 18.17GB \\
    \bottomrule
    \end{tabular}
    \label{table:chair-efficiency}
\vspace{-12pt}
\end{minipage}
\hfill
\begin{minipage}{0.48\linewidth}
\renewcommand{\arraystretch}{1.0}
    \centering
    \scriptsize
    \caption{Module Efficiency on CHAIR}
\vspace{-6pt}

    \begin{tabular}{lcc}
    \toprule
    Module  & T (s/sample)$\downarrow$ & Mem$\downarrow$ \\ \hline
    Vanilla                        & 2.59 & 15.69GB \\
    w/ Mitigate Statistical Bias    & 4.64 & 16.56GB \\
    w/ Reduce Inherent Bias         & 2.63 & 16.50GB \\
    w/ Address Vulnerability        & 7.30 & 18.17GB \\
    \rowcolor[HTML]{C0C0C0}
    Ours (All Modules)             & 7.34 & 18.17GB \\
    \bottomrule
    \end{tabular}
    \label{table:ablation-modules}
\vspace{-12pt}
\end{minipage}
\end{table}


==> iclr2026/tables/mme-and-ablation.tex <==
\begin{table}[t]
\centering
\begin{minipage}{0.48\linewidth}
\renewcommand{\arraystretch}{1.0}  
    \centering
    \scriptsize
    \caption{MME Full Set Evaluation}
\vspace{-6pt}
    \begin{tabular}{cccc}
    \toprule
    Method  & Perception$\uparrow$       & Cognition$\uparrow$       & Total Score$\uparrow$     \\ \hline
    Vanilla & 1279.2           & 352.9           & 1632.1          \\
    VCD     & 1363.9           & \textbf{353.2}  & 1717.1          \\
    OPERA   & 1413.0           & 304.2           & 1717.2          \\
    \rowcolor[HTML]{C0C0C0} 
    Ours    & \textbf{1473.0}  & 337.8           & \textbf{1810.8} \\ \bottomrule
    \end{tabular}
    \label{table:mme-full}
\vspace{-12pt}
\end{minipage}
\hfill
\begin{minipage}{0.48\linewidth}
\renewcommand{\arraystretch}{1.0}  
    \centering
    \scriptsize
    \caption{Module Ablation on CHAIR}
\vspace{-6pt}
    \begin{tabular}{lcc}
    \toprule
    \multicolumn{1}{c}{Module}                              & $C_S$$\downarrow$  & $C_I$$\downarrow$      \\
    \hline
    Vanilla LLaVA-1.5                                        & 48.8          & 14.2          \\
    \quad\quad+ adaptive plausibility constraint             & 50.2          & 13.8          \\
    \hline
    \quad\quad+ address vulnerability (Ours)                       & 46.4          & 12.8          \\
    
    \quad\quad+ mitigate statistical bias (Ours)                   & 40.4          & 11.0          \\
    
    \quad\quad+ reduce inherent bias (Ours)                        & \textbf{36.6} & \textbf{10.3} \\
    \bottomrule
    
    \end{tabular}
    \label{table:ablation}
\vspace{-12pt}
\end{minipage}
\end{table}


==> iclr2026/tables/module-ablation.tex <==
\begingroup
\renewcommand{\arraystretch}{1.0}  
\begin{table}[t]
% \small
\centering
\caption{Module Ablation on CHAIR using LLaVA-1.5}
\begin{tabular}{lcc}
\toprule
\multicolumn{1}{c}{Module}                              & $C_S$$\downarrow$  & $C_I$$\downarrow$      \\
\hline
Vanilla LLaVA-1.5                                        & 48.8          & 14.2          \\
\quad\quad+ adaptive plausibility constraint             & 50.2          & 13.8          \\
\hline
\quad\quad+ address vulnerability (Ours)                       & 46.4          & 12.8          \\

\quad\quad+ mitigate statistical bias (Ours)                   & 40.4          & 11.0          \\

\quad\quad+ reduce inherent bias (Ours)                        & \textbf{36.6} & \textbf{10.3} \\
\bottomrule

\end{tabular}
\label{table:ablation}
\end{table}
\endgroup

==> tables/CHAIR-trainingfree.tex <==
% \begingroup
% \begin{table}[t]
% % \renewcommand{\arraystretch}{1.1}  
% \renewcommand{\arraystretch}{1.0}  
% % \small
% \centering
% \caption{Comparison with Training-Free Methods on CHAIR}
% \begin{tabular}{ccccccc}
% \toprule
%                          & \multicolumn{2}{c}{LLaVA-1.5} & \multicolumn{2}{c}{InstructBLIP} & \multicolumn{2}{c}{Qwen-VL} \\
% \multirow{-2}{*}{Method} & $C_S$$\downarrow$  & $C_I$$\downarrow$   & $C_S$$\downarrow$        & $C_I$$\downarrow$       & $C_S$$\downarrow$     & $C_I$$\downarrow$     \\ \hline
% Vanilla                  & 48.8                 & 14.2                  & 54.6                       & 24.8                      & 49.2                    & 13.1         \\
% VCD                      & 46.8                 & 13.2                  & 44.0                       & 13.6                      & 46.4                    & 11.9         \\
% OPERA                    & 44.6                 & 12.8                  & 46.4                       & 14.2                      & 34.6                    & 9.5          \\
% \rowcolor[HTML]{C0C0C0} 
% CCD (Ours)                     & \textbf{36.6} & \textbf{10.3} & \textbf{40.4}   & \textbf{10.9}  & \textbf{28.9}            & \textbf{9.2}             \\ 
% \bottomrule
% \end{tabular}
% \label{table:chair}
% \end{table}
% \endgroup


==> tables/GPT4o-aid-eval.tex <==
\begingroup
\renewcommand{\arraystretch}{1.0}  
\begin{table}[t]
\centering
\caption{GPT-4o Assisted Hallucination Evaluation}
\begin{tabular}{ccccccc}
\toprule
                         & \multicolumn{2}{c}{LLaVA-1.5}        & \multicolumn{2}{c}{InstructBLIP}      & \multicolumn{2}{c}{Qwen-VL} \\
\multirow{-2}{*}{Method} & $C$$\uparrow$    & $D$$\uparrow$     & $C$$\uparrow$     & $D$$\uparrow$     & $C$$\uparrow$ & $D$$\uparrow$ \\ \hline
Vanilla                  & 4.9              & 5.0               & 4.2               & 4.2               &  6.2             & 4.6              \\
VCD                      & 5.5              & 5.5               & 5.1               & \textbf{5.5}      &  6.5             & 5.7              \\
OPERA                    & 5.6              & 6.0               & 5.3               & 5.2               &  6.5             & 5.6                  \\
\rowcolor[HTML]{C0C0C0} 
CCD (Ours)                      & \textbf{6.2}     & \textbf{6.1}      & \textbf{5.6}      & 5.3               &  \textbf{6.9}    & \textbf{5.8}              \\ 
\bottomrule
\end{tabular}
\label{table:gpt4o-eval}
\end{table}
\endgroup


==> tables/MME-full.tex <==
\begin{table}[t]
\centering

\caption{LVLM General Evaluation on MME Dataset}
\begin{tabular}{cccc}
\toprule
Method  & Perception$\uparrow$       & Cognition$\uparrow$       & Total Score$\uparrow$     \\ \hline
Vanilla & 1279.2           & 352.9           & 1632.1          \\
VCD     & 1363.9           & \textbf{353.2}  & 1717.1          \\
OPERA   & 1413.0           & 304.2           & 1717.2          \\
\rowcolor[HTML]{C0C0C0} 
CCD (Ours)    & \textbf{1473.0}  & 337.8           & \textbf{1810.8} \\ \bottomrule
\end{tabular}
\label{table:mme-full}
\end{table}


==> tables/MMhal.tex <==
\begin{table}[t]
\centering
\scriptsize
\renewcommand{\arraystretch}{1.0}
\caption{MMHal-Bench Evaluation (LLaVA-1.5 7B)}
\vspace{-4pt}

{\color{blue}
\begin{tabular}{lcccccccccc}
\toprule
\textbf{Method} &
\textbf{Overall}$\uparrow$ &
\textbf{Hallucination}$\downarrow$ &
\textbf{Attribute}$\uparrow$ &
\textbf{Adversarial}$\uparrow$ &
\textbf{Comparison}$\uparrow$ &
\textbf{Counting}$\uparrow$ &
\textbf{Relation}$\uparrow$ &
\textbf{Environment}$\uparrow$ &
\textbf{Holistic}$\uparrow$ &
\textbf{Other}$\uparrow$ \\
\midrule

Vanilla 
& 2.21 
& 0.70 
& \textbf{2.75}
& \textbf{2.00}
& 2.50
& 2.50
& 1.67
& 2.17
& 1.83
& 2.25 \\

\rowcolor[HTML]{C0C0C0}
Ours    
& \textbf{2.65}
& \textbf{0.61}
& 2.42
& 1.83
& \textbf{2.58}
& \textbf{2.67}
& \textbf{2.83}
& \textbf{3.92}
& \textbf{2.08}
& \textbf{2.83} \\

\bottomrule
\end{tabular}
}
\end{table}


==> tables/POPE-traingfree.tex <==
\begingroup
\begin{table*}[ht]
\centering
\label{table:pope}
\begin{tabular}{ccl|cccccc|cc}
\toprule
                                &                           & \multicolumn{1}{c}{}                           & \multicolumn{2}{c}{Random}                                                    & \multicolumn{2}{c}{Popular}                                                   & \multicolumn{2}{c}{Adversarial}                                               & \multicolumn{2}{c}{Average}                                                   \\
\cline{4-5} \cline{6-7} \cline{8-9} \cline{10-11}
                                
\multirow{-2}{*}{LVLM}          & \multirow{-2}{*}{Dataset} & \multicolumn{1}{c}{\multirow{-2}{*}{Method}} & Acc$\uparrow$                                  & F1$\uparrow$                                   & Acc$\uparrow$                                  & F1$\uparrow$                                   & Acc$\uparrow$                                  & \multicolumn{1}{c}{F1$\uparrow$}                                   & Acc$\uparrow$                                  & F1$\uparrow$                                   \\
\cline{1-11}
                                &                           & Vanilla\cite{llava}                                        & 83.2                                  & 81.3                                  & 81.8                                  & 80.0                                  & 78.9                                  & 77.5                                  & 81.3                                  & 79.6                                  \\
                                &                           & VCD\cite{VCD}                                            & 87.7                                  & 87.1                                  & 85.3                                  & 85.0                                  & 80.8                                  & 81.3                                  & 84.6                                  & 84.4                                  \\
                                &                           & OPERA\cite{OPERA}                                          & 89.1                                  & 89.0                                  & 86.0                                  & 86.3                                  & 79.1                                  & 80.9                                  & 84.7                                  & 85.4                                  \\
                                & \multirow{-4}{*}{COCO}    & \cellcolor[HTML]{C0C0C0}Ours                   & \cellcolor[HTML]{C0C0C0}\textbf{91.3} & \cellcolor[HTML]{C0C0C0}\textbf{91.1} & \cellcolor[HTML]{C0C0C0}\textbf{87.4} & \cellcolor[HTML]{C0C0C0}\textbf{87.6} & \cellcolor[HTML]{C0C0C0}\textbf{82.5} & \cellcolor[HTML]{C0C0C0}\textbf{83.6} & \cellcolor[HTML]{C0C0C0}\textbf{87.0} & \cellcolor[HTML]{C0C0C0}\textbf{87.4} \\
\cline{1-11}
                                &                           & Vanilla\cite{instructblip}                                        & 80.7                                  & 80.4                                  & 78.2                                  & 78.3                                  & 75.8                                  & 76.5                                  & 78.2                                  & 78.4                                  \\
                                &                           & VCD\cite{VCD}                                            & 84.5                                  & 83.6                                  & 81.4                                  & 81.0                                  & 79.5                                  & 79.5                                  & 81.8                                  & 81.3                                  \\
                                &                           & OPERA\cite{OPERA}                                          & \textbf{89.8}                         & \textbf{89.6}                         & 83.4                                  & 84.0                                  & 80.7                                  & 81.8                                  & 84.6                                  & \textbf{85.1}                         \\
                                & \multirow{-4}{*}{COCO}    & \cellcolor[HTML]{C0C0C0}Ours                   & \cellcolor[HTML]{C0C0C0}88.6          & \cellcolor[HTML]{C0C0C0}88.0          & \cellcolor[HTML]{C0C0C0}\textbf{84.9} & \cellcolor[HTML]{C0C0C0}\textbf{84.6} & \cellcolor[HTML]{C0C0C0}\textbf{81.8} & \cellcolor[HTML]{C0C0C0}\textbf{82.1} & \cellcolor[HTML]{C0C0C0}\textbf{85.1} & \cellcolor[HTML]{C0C0C0}84.9          \\
\cline{1-11}
                                &                           & Vanilla\cite{qwen-vl}                                        & 84.7                                  & 82.6                                  & 84.1                                  & 82.0                                  & 82.2                                  & 80.3                                  & 83.6                                  & 81.6                                  \\
                                &                           & VCD\cite{VCD}                                            & 88.6                                  & 87.8                                  & 87.1                                  & 86.4                                  & 84.2                                  & 83.9                                  & 86.6                                  & 86.0                                  \\
                                &                           & OPERA\cite{OPERA}                                          & 86.1                                  & 84.2                                  & 85.7                                  & 83.8                                  & 83.9                                  & 82.1                                  & 85.2                                  & 83.3                                  \\
                                & \multirow{-4}{*}{COCO}    & \cellcolor[HTML]{C0C0C0}Ours                   & \cellcolor[HTML]{C0C0C0}              & \cellcolor[HTML]{C0C0C0}              & \cellcolor[HTML]{C0C0C0}              & \cellcolor[HTML]{C0C0C0}              & \cellcolor[HTML]{C0C0C0}              & \cellcolor[HTML]{C0C0C0}              & \cellcolor[HTML]{C0C0C0}              & \cellcolor[HTML]{C0C0C0}              \\ 
\bottomrule
\end{tabular}
\caption{Comparison with Training-Free Methods on POPE}
\end{table*}
\endgroup


==> tables/module-ablation.tex <==
\begingroup
\renewcommand{\arraystretch}{1.0}  
\begin{table}[t]
% \small
\centering
\caption{Module Ablation on CHAIR using LLaVA-1.5}
\begin{tabular}{lcc}
\toprule
\multicolumn{1}{c}{Module}                              & $C_S$$\downarrow$  & $C_I$$\downarrow$      \\
\hline
Vanilla LLaVA-1.5                                        & 48.8          & 14.2          \\
\quad\quad+ adaptive plausibility constraint             & 50.2          & 13.8          \\
\hline
\quad\quad+ address vulnerability (Ours)                       & 46.4          & 12.8          \\

\quad\quad+ mitigate statistical bias (Ours)                   & 40.4          & 11.0          \\

\quad\quad+ reduce inherent bias (Ours)                        & \textbf{36.6} & \textbf{10.3} \\
\bottomrule

\end{tabular}
\label{table:ablation}
\end{table}
\endgroup
